A generative approach to frame-level multi-competitor races

Multi-competitor races often feature complicated within-race strategies that are difficult to capture when training data on race outcome level data. Further, models which do not account for such strategic effects may suffer from confounded inferences and predictions. In this work we develop a general generative model for multi-competitor races which allows analysts to explicitly model certain strategic effects such as changing lanes or drafting and separate these impacts from competitor ability. The generative model allows one to simulate full races from any real or created starting position which opens new avenues for attributing value to within-race actions and to perform counter-factual analyses. This methodology is sufficiently general to apply to any track based multi-competitor races where both tracking data is available and competitor movement is well described by simultaneous forward and lateral movements. We apply this methodology to one-mile horse races using data provided by the New York Racing Association (NYRA) and the New York Thoroughbred Horsemen's Association (NYTHA) for the Big Data Derby 2022 Kaggle Competition. This data features granular tracking data for all horses at the frame-level (occurring at approximately 4hz). We demonstrate how this model can yield new inferences, such as the estimation of horse-specific speed profiles which vary over phases of the race, and examples of posterior predictive counterfactual simulations to answer questions of interest such as starting lane impacts on race outcomes.

==> alt-bib.tex <==
\begin{thebibliography}{10}

\bibitem{goog}
Google earth.
\newblock \url{https://earth.google.com/}.
\newblock date accessed: 2022-08-30.

\bibitem{carpenter2017stan}
Bob Carpenter, Andrew Gelman, Matthew~D Hoffman, Daniel Lee, Ben Goodrich,
  Michael Betancourt, Marcus~A Brubaker, Jiqiang Guo, Peter Li, and Allen
  Riddell.
\newblock Stan: A probabilistic programming language.
\newblock {\em Journal of statistical software}, 76, 2017.

\bibitem{cervone2016multiresolution}
Daniel Cervone, Alex D’Amour, Luke Bornn, and Kirk Goldsberry.
\newblock A multiresolution stochastic process model for predicting basketball
  possession outcomes.
\newblock {\em Journal of the American Statistical Association},
  111(514):585--599, 2016.

\bibitem{che2022athlete}
Jonathan Che and Mark Glickman.
\newblock Athlete rating in multi-competitor games with scored outcomes via
  monotone transformations.
\newblock {\em arXiv preprint arXiv:2205.10746}, 2022.

\bibitem{blender}
Blender~Online Community.
\newblock {\em Blender - a 3D modelling and rendering package}.
\newblock Blender Foundation, Stichting Blender Foundation, Amsterdam, 2018.

\bibitem{fahrmeir1994dynamic}
Ludwig Fahrmeir and Gerhard Tutz.
\newblock Dynamic stochastic models for time-dependent ordered paired
  comparison systems.
\newblock {\em Journal of the American Statistical Association},
  89(428):1438--1449, 1994.

\bibitem{fernandez2021framework}
Javier Fern{\'a}ndez, Luke Bornn, and Daniel Cervone.
\newblock A framework for the fine-grained evaluation of the instantaneous
  expected value of soccer possessions.
\newblock {\em Machine Learning}, 110(6):1389--1427, 2021.

\bibitem{glickman1999parameter}
Mark~E Glickman.
\newblock Parameter estimation in large dynamic paired comparison experiments.
\newblock {\em Journal of the Royal Statistical Society Series C: Applied
  Statistics}, 48(3):377--394, 1999.

\bibitem{glickman2001dynamic}
Mark~E Glickman.
\newblock Dynamic paired comparison models with stochastic variances.
\newblock {\em Journal of Applied Statistics}, 28(6):673--689, 2001.

\bibitem{glickman2015stochastic}
Mark~E Glickman and Jonathan Hennessy.
\newblock A stochastic rank ordered logit model for rating multi-competitor
  games and sports.
\newblock {\em Journal of Quantitative Analysis in Sports}, 11(3):131--144,
  2015.

\bibitem{glickman2005state}
Mark~E Glickman and Hal~S Stern.
\newblock A state-space model for national football league scores.
\newblock In {\em Anthology of statistics in sports}, pages 23--33. SIAM, 2005.

\bibitem{harville1973assigning}
David~A Harville.
\newblock Assigning probabilities to the outcomes of multi-entry competitions.
\newblock {\em Journal of the American Statistical Association},
  68(342):312--316, 1973.

\bibitem{henery1981permutation}
RJ~Henery.
\newblock Permutation probabilities as models for horse races.
\newblock {\em Journal of the Royal Statistical Society Series B: Statistical
  Methodology}, 43(1):86--91, 1981.

\bibitem{jasak2009openfoam}
Hrvoje Jasak.
\newblock Openfoam: Open source cfd in research and industry.
\newblock {\em International Journal of Naval Architecture and Ocean
  Engineering}, 1(2):89--94, 2009.

\bibitem{kovalchik2020extension}
Stephanie Kovalchik.
\newblock Extension of the elo rating system to margin of victory.
\newblock {\em International Journal of Forecasting}, 36(4):1329--1341, 2020.

\bibitem{luce1959individual}
R~Duncan Luce.
\newblock Individual choice behavior.
\newblock 1959.

\bibitem{aqu}
New York Racing~Association (NYRA).
\newblock Aqueduct race track: Top jockeys.
\newblock \url{https://www.nyra.com/aqueduct/leaders/jockeys}.
\newblock date accessed: 2022-11-06.

\bibitem{bel}
New York Racing~Association (NYRA).
\newblock Belmont: Top jockeys.
\newblock \url{https://www.nyra.com/belmont/leaders/jockeys}.
\newblock date accessed: 2022-11-06.

\bibitem{sar}
New York Racing~Association (NYRA).
\newblock Saratoga race course: Top jockeys.
\newblock \url{https://www.nyra.com/saratoga/leaders/jockeys}.
\newblock date accessed: 2022-11-06.

\bibitem{bdd}
New York Racing~Association (NYRA) and New York Thoroughbred
  Horsemen’s~Association (NYTHA).
\newblock Big data derby.
\newblock
  \url{https://www.kaggle.com/competitions/big-data-derby-2022/overview}.

\bibitem{plackett1975analysis}
Robin~L Plackett.
\newblock The analysis of permutations.
\newblock {\em Journal of the Royal Statistical Society Series C: Applied
  Statistics}, 24(2):193--202, 1975.

\bibitem{spence2012speed}
Andrew~J Spence, Andrew~S Thurman, Michael~J Maher, and Alan~M Wilson.
\newblock Speed, pacing strategy and aerodynamic drafting in thoroughbred horse
  racing.
\newblock {\em Biology letters}, 8(4):678--681, 2012.

\bibitem{vanbrummelen2012}
Glen Van~Brummelen.
\newblock Heavenly mathematics: The forgotten art of spherical trigonometry.
\newblock {\em Princeton University Press}, 2012.

\bibitem{loo}
Aki Vehtari, Jonah Gabry, Mans Magnusson, Yuling Yao, Paul-Christian Bürkner,
  Topi Paananen, and Andrew Gelman.
\newblock loo: Efficient leave-one-out cross-validation and waic for bayesian
  models, 2022.
\newblock R package version 2.5.1.

\bibitem{wang2021shape}
Wenjie Wang and Jun Yan.
\newblock Shape-restricted regression splines with r package splines2.
\newblock {\em Journal of Data Science}, 19(3), 2021.

\bibitem{de1978practical}
Carl De Boor.
\newblock A practical guide to splines.
\newblock {\em springer-verlag New York}, 1978.

\bibitem{dierckx1995curve}
Paul Dierckx.
\newblock Curve and surface fitting with splines.
\newblock {\em Oxford University Press}, 1995.

\end{thebibliography}


==> custom_commands.tex <==
\newcommand{\y}{\boldsymbol{y}}
\newcommand{\ty}{\tilde{\y}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\lat}{\text{lat}}
\newcommand{\f}{\text{for}}
\newcommand{\bx}{\boldsymbol{X}}
\newcommand{\yf}{\ty^{\f}}
\newcommand{\yl}{\ty^{\lat}}
\newcommand{\tl}{\btheta^{\lat}}
\newcommand{\tf}{\btheta^{\f}}
\newcommand{\Xl}{\bx^{\lat}}
\newcommand{\Xf}{\bx^{\f}}
\newcommand{\I}{\boldsymbol{I}}


